Adaptive Neural Compilation

This paper proposes an adaptive neural-compilation framework to address the problem of efficient program learning. Traditional code optimisation strategies used in compilers are based on applying pre-specified set of transformations that make the code faster to execute without changing its semantics. In contrast, our work involves adapting programs to make them more efficient while considering correctness only on a target input distribution. Our approach is inspired by the recent works on differentiable representations of programs. We show that it is possible to compile programs written in a low-level language to a differentiable representation. We also show how programs in this representation can be optimised to make them efficient on a target distribution of inputs. Experimental results demonstrate that our approach enables learning specifically-tuned algorithms for given data distributions with a high success rate.

==> schema.tex <==



\begin{figure}

  \begin{center}
    \usetikzlibrary{decorations.pathreplacing,calc,matrix,circuits.logic.US,positioning,matrix, fit}

    \begin{tikzpicture}[circuit logic US,
      tiny circuit symbols,
      every circuit symbol/.style={fill=white,draw, logic gate input sep=2mm}
      ]

      % Machine
      {
        % Registers before the machine
        \matrix (before-reg)[matrix of nodes,row sep=-\pgflinewidth,nodes={rectangle,draw}]
        {
          $r_1$  \\
          $r_2$  \\
          $r_3$  \\
          $r_4$  \\
        };
        \node[rectangle, draw, thick, above=0cm of before-reg] (before-reg-inst) {$r_{I}$};
        \node[fit=(before-reg)(before-reg-inst)](registers-before){};


        % Execution of the machine
        \node[draw, circle, above right = -1cm and 2cm of registers-before] (arg1) {Arg 1};
        \node[draw, circle, below = of arg1, node distance = 0.5 and 3] (arg2) {Arg 2};
        \node[fit=(arg1)(arg2)](in-args){};
        \node[or gate, draw, right = 1.5cm of in-args, text height = 0.7cm] (module) {};
        \node[above =-0.6cm of module] {Inst};
        \node[draw, circle, right = 2cm of module] (out) {Out};
        \node[fit=(in-args)(module)(out)](execution){};

        % Registers after the machine
        \matrix (after-reg)[matrix of nodes,row sep=-\pgflinewidth,nodes={rectangle,draw}, right = 10cm of before-reg]
        {
          $r_1$  \\
          $r_2$  \\
          $r_3$  \\
          $r_4$  \\
        };
        \node[rectangle, draw, thick, above=0cm of after-reg] (after-reg-inst) {$r_{I}$};
        \node[fit=(after-reg)(after-reg-inst)](registers-after){};


        % Borders
        \node[fit=(registers-before)(execution)(registers-after)](machine-content){};
        \draw[ultra thick, draw=black, fill=gray, opacity=0.2]
        (machine-content.north east) -- (machine-content.north west) --
        (machine-content.south west) -- (machine-content.south east) -- cycle;

        % Label
        \node[above left = 0.2cm and 0.2cm of machine-content.south east] (machine-label) {\Large Machine};
      }

      % Controller
      \node[draw, rectangle, above = of machine-content]  (Controller) {\LARGE Controller};

      % Memory
      \tikzset{memorycell/.style={draw,rectangle, text width = 0.5cm, text height = 0.5cm}}
      \matrix[matrix of nodes, nodes in empty cells,
      row sep=-0.5\pgflinewidth,
      column sep=-0.5\pgflinewidth,
      below = of machine-content,
      nodes={memorycell}] (memory) {
        & & & & &  & & & & & \\
      };
      \node[below = 0cm of memory] (memory-label){\large Memory Tape};

      % All arrows
      {
        % Instruction register to controller
        \draw[->, thick] (before-reg-inst.north) to[in=90, out=90] node[midway, above, circle, draw]{1} (Controller.north);

        % Parameters of the controller to the args, instruct and out node
        % Intermediary points to have nicer arrows
        \draw[-, dotted, thick] (Controller.south) to[out=-90, in=90] node[midway, above right, circle, draw, solid]{2} ([xshift=3cm]machine-content.north);
        \draw[-, dotted, thick] ([xshift=3cm]machine-content.north) to [out=-90, in=0] ([xshift=1cm,yshift=-0.8cm]machine-content.north);
        % To the correct place
        \draw[->, dotted, thick] ([xshift=1cm,yshift=-0.8cm]machine-content.north) to[out=180, in=0] (arg1.north east);
        \draw[->, dotted, thick] ([xshift=1cm,yshift=-0.8cm]machine-content.north) to[out=180, in=90] (arg2.north);
        \draw[->, dotted, thick] ([xshift=1cm,yshift=-0.8cm]machine-content.north) to[out=180, in=90] (module.north);
        \draw[->, dotted, thick] ([xshift=3cm]machine-content.north) to[out=-90, in=90] (out.north);

        % Execution with the parameters fixed
        \draw[->, dashed, thick] (before-reg-2-1.south east) to node[midway, below, circle, draw, solid]{3} (arg1);
        \draw[->, dashed, thick] (before-reg-2-1.south east) to (arg2);
        \draw[->, dashed, thick] (arg1.east) to (module.input 1);
        \draw[->, dashed, thick] (arg2.east) to (module.input 2);
        \draw[->, dashed, thick] (module.output) to (out.west);
        \draw[->, dashed, thick] (out.east) to (after-reg-2-1.south west);
        \draw[->, dashed, thick] (module) to[bend left=20] (memory);
        \draw[<-, dashed, thick] (module) to[bend right=20] (memory);
        \draw[->, dashed, thick] (before-reg-inst) to[bend right=5] ([yshift=-0.1cm]module.input 1);
        \draw[->, dashed, thick] (module.output) to[bend left=15, out=0] (after-reg-inst);


      }

    \end{tikzpicture}
  \end{center}
  \caption{\label{fig:schema}Execution of a timestep.
    \textbf{1}\textit{(solid)} The special instruction registers is fed as input to the controller.
    \textbf{2}\textit{(dotted)} The controllers computes the parameters that specify the execution of the machine: how are elements of the registers combined as arguments, which mix of instructions will be executed and which registers will receive the results.
    \textbf{3}\textit{(dashed)} The arguments are computed, all operations are executed simultaneously and their outputs are combined according to the parameters and stored in the targeted registers. The memory tape is updated.}
\end{figure}

